Q-Mask: Query-driven Causal Masks for Text Anchoring in OCR-Oriented Vision-Language Models

Optical Character Recognition (OCR) is increasingly regarded as a foundational capability for modern vision-language models (VLMs), enabling them not only to read text in images but also to support downstream reasoning in real-world visual question answering (VQA). However, practical applications further require reliable text anchors, i.e., accurately grounding queried text to its corresponding spatial region. To systematically evaluate this capability, we introduce TextAnchor-Bench (TABench), a benchmark for fine-grained text-region grounding, which reveals that both general-purpose and OCR-specific VLMs still struggle to establish accurate and stable text anchors. To address this limitation, we propose Q-Mask, a precise OCR framework built upon a causal query-driven mask decoder (CQMD). Inspired by chain-of-thought reasoning, Q-Mask performs causal visual decoding that sequentially generates query-conditioned visual masks before producing the final OCR output. This visual CoT paradigm disentangles where the text is from what the text is, enforcing grounded evidence acquisition prior to recognition and enabling explicit text anchor construction during inference. To train CQMD, we construct TextAnchor-26M, a large-scale dataset of image-text pairs annotated with fine-grained masks corresponding to specific textual elements, encouraging stable text-region correspondences and injecting strong spatial priors into VLM training. Extensive experiments demonstrate that Q-Mask substantially improves text anchoring and understanding across diverse visual scenes.

==> main/tables/benchmark_1.tex <==
\begin{tabular}{@{}l cc@{}}
\toprule
\textbf{Category} & \textbf{Region-to-Text} & \textbf{Text-to-Region} \\
\midrule
SceneText       & 1,380 & 1,380 \\
Receipt         & 280   & 280   \\
Ticket          & 230   & 230   \\
Warehouse slip  & 195   & 195   \\
Report          & 140   & 140   \\
document        & 135   & 135   \\
Book            & 105   & 105   \\
Poster          & 90    & 90    \\
Notice          & 60    & 60    \\
PriceTag        & 40    & 40    \\
Invoice         & 40    & 40    \\
Certificate     & 30    & 30    \\
\midrule
\textbf{Overall} & \textbf{2,725} & \textbf{2,725} \\
\bottomrule
\end{tabular}

==> main/tables/benchmark_2.tex <==
\begin{tabular}{@{}ll r@{}}
\toprule
\multicolumn{2}{@{}l}{\textbf{Distribution Metric}} & \textbf{Count} \\
\midrule
\multirow{4}{*}{\textbf{Source Dataset}} 
& HierText & 3,348 \\
& SRVD & 1,784 \\
& CDLA & 270 \\
& ICDAR2015 & 48 \\
\midrule
\multirow{2}{*}{\textbf{Lang: Region-to-Text}} 
& English (EN) & 2,095 \\
& ZH / Mixed & 630 \\
\cmidrule(l){2-3}
\multirow{2}{*}{\textbf{Lang: Text-to-Region}} 
& English (EN) & 2,017 \\
& ZH / Mixed & 708 \\
\midrule
\multirow{3}{*}{\textbf{Granularity}} 
& Line-level & 5,062 \\
& Word-level & 262 \\
& Paragraph & 126 \\
\bottomrule
\end{tabular}

==> main/tables/empirical_noise.tex <==
\begin{tabular}{@{} l c cc cc @{}}
  \toprule
  & \textbf{E2E Metrics} & \multicolumn{2}{c}{\textbf{Box-level Metrics}} & \multicolumn{2}{c}{\textbf{Character-level Errors}} \\
  \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(l){5-6}
  \textbf{Dataset} & \textbf{Accuracy} & \textbf{Recall} & \textbf{Precision} & \textbf{CER} & \textbf{Norm. Breakdown} \\
   & \textbf{(\%)} & \textbf{(\%)} & \textbf{(\%)} & \textbf{(\%)} & \textbf{Ins / Del / Sub (\%)} \\
  \midrule
  HireText & 29.72 & 47.08 & 70.07 & 53.50 & 27.2 / 69.1 / \phantom{0}3.7 \\
  SynthZh  & 61.38 & 79.93 & 92.48 & 17.94 & 24.6 / 51.9 / 23.5 \\
  SynthEn  & 59.87 & 90.00 & 97.32 & 25.47 & \phantom{0}3.5 / 35.0 / 61.6 \\
  \midrule
  \textbf{Overall}  & \textbf{40.83} & \textbf{60.69} & \textbf{80.72} & \textbf{44.14} & \textbf{24.4 / 64.5 / 11.1} \\
  \bottomrule
\end{tabular}

==> main/tables/noise_injection_abaltion.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation of Stochastic Prior Injection (SPI) at the 5M checkpoint. Evaluated under strict zero-shot conditions, standard training without our prior injection acts as a "lazy guesser" (inflating F1 but failing in exact pointing). SPI forces rigorous visual verification, directly resulting in superior exact reading (Acc), halved hallucinations (CER), strictly better first-try spatial intuition (QSR@1), and a higher overall Omni-Alignment Index.}
\label{tab:spi_ablation}
\resizebox{\linewidth}{!}{
\begin{tabular}{l cccc c}
\toprule
\multirow{2}{*}{\textbf{Training Setting (5M)}} & \multicolumn{2}{c}{\textbf{T1: Region-to-Text}} & \multicolumn{2}{c}{\textbf{T2: Text-to-Region}} & \multirow{2}{*}{\textbf{OAI}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& \textbf{Acc} $\uparrow$ & \textbf{CER} $\downarrow$ & \textbf{QSR@1} $\uparrow$ & \textbf{F1} $\uparrow$ & \\
\midrule
Standard Training (No Prior Injection) & 46.53 & 1.17 & 49.13 & \textbf{43.09} & 46.32 \\
\midrule
\rowcolor{gray!10}
\textbf{w/ SPI (Ours)} & \textbf{49.90} & \textbf{0.60} & \textbf{54.00} & 35.00 & \textbf{47.20} \\
\bottomrule
\end{tabular}
}
\end{table}

==> main/tables/stage_correlation.tex <==
\begin{table*}[t]
\centering
\caption{Evolution of model capabilities across the training trajectory. The Omni-Alignment Index (OAI) elegantly captures the training dynamics, including the "alignment shock" at 3M. Crucially, as the OAI stabilizes and monotonically increases from 4M to 30M, we observe a perfect positive correlation with the explosive gains in Stage-2 downstream reasoning tasks.}
\label{tab:correlation_trajectory}
\resizebox{\textwidth}{!}{
\begin{tabular}{l | cccc c | ccccc}
\toprule
\multirow{2}{*}{\textbf{Checkpoint}} & \multicolumn{5}{c|}{\textbf{Stage-1: FineGround Probe}} & \multicolumn{5}{c}{\textbf{Stage-2: Downstream Tasks}} \\
\cmidrule(lr){2-6} \cmidrule(l){7-11}
& \textbf{T1 Acc} & \textbf{T1 CER} & \textbf{T2 QSR@1} & \textbf{T2 F1} & \cellcolor{gray!15}\textbf{OAI} & \textbf{ChartQA} & \textbf{DocVQA} & \textbf{InfoVQA} & \textbf{TextVQA} & \textbf{OCRBench} \\
\midrule
Baseline & 0.51  & 2.10 & 18.40 & 14.89 & \cellcolor{gray!15} 8.57  & 80.44 & 92.65 & 77.1 & 79.3 & 797 \\
\midrule
Ours - 1M  & 42.20 & 1.10 & 49.67 & 22.70 & \cellcolor{gray!15} 39.19 & - & - & - & - & - \\
Ours - 2M  & 46.49 & 8.75 & 56.10 & 26.95 & \cellcolor{gray!15} 44.00 & - & - & - & - & - \\
Ours - 3M  & 42.97 & 0.52 & 46.12 & 16.69 & \cellcolor{gray!15} 37.18 & - & - & - & - & - \\
Ours - 4M  & 46.86 & 2.32 & 57.17 & 34.91 & \cellcolor{gray!15} 46.45 & - & - & - & - & - \\
Ours - 5M  & \textbf{49.90} & \textbf{0.60} & 54.00 & 35.00 & \cellcolor{gray!15} 47.20 & 86.4 & 93.4 & 76.2 & 83.6 & 830 \\
Ours - 10M & 47.90 & 1.07 & 52.20 & 45.19 & \cellcolor{gray!15} 48.30 & 86.6 & 93.6 & 79.8 & 88.5 & 826 \\
Ours - 30M & 45.40 & 2.00 & \textbf{57.40} & \textbf{51.40} & \cellcolor{gray!15} \textbf{49.90} & \textbf{87.2} & \textbf{93.5} & \textbf{78.7} & \textbf{88.5} & \textbf{855} \\
\bottomrule
\end{tabular}
}
\end{table*}
